Secure Metric Learning via Differential Pairwise Privacy

Distance Metric Learning (DML) has drawn much attention over the last two decades. A number of previous works have shown that it performs well in measuring the similarities of individuals given a set of correctly labeled pairwise data by domain experts. These important and precisely-labeled pairwise data are often highly sensitive in real world (e.g., patients similarity). This paper studies, for the first time, how pairwise information can be leaked to attackers during distance metric learning, and develops differential pairwise privacy (DPP), generalizing the definition of standard differential privacy, for secure metric learning. Unlike traditional differential privacy which only applies to independent samples, thus cannot be used for pairwise data, DPP successfully deals with this problem by reformulating the worst case. Specifically, given the pairwise data, we reveal all the involved correlations among pairs in the constructed undirected graph. DPP is then formalized that defines what kind of DML algorithm is private to preserve pairwise data. After that, a case study employing the contrastive loss is exhibited to clarify the details of implementing a DPP-DML algorithm. Particularly, the sensitivity reduction technique is proposed to enhance the utility of the output distance metric. Experiments both on a toy dataset and benchmarks demonstrate that the proposed scheme achieves pairwise data privacy without compromising the output performance much (Accuracy declines less than 0.01 throughout all benchmark datasets when the privacy budget is set at 4).

==> IEEE TIFS P3DML-compiled/R1.tex <==
% !TEX root = response.tex

\newpage
\subsection*{To Reviewer \#1}
Thank you very much for such valuable comments. Below is a report for how we address your concerns. 
%% -------------------------------------------------------------------------
\begin{shaded}
	\noindent \textbf{Comment $1.1$}
	In Introduction Section, the authors did not mention graphs. However, in Section III, the Notation and the definition are based on the graph structure. Please introduce the graph structure to readers in the Introduction Section. 
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} We have introduced the graph structure in the 5th paragraph of the Introduction section as suggested by the reviewer. Given a number of pairwise data, we can describe them on a indirect graph. Then the pairwise information can be naturally encoded on edges. This is the base of our method, and we thank the reviewer for pointing this out.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $1.2$}
	In the experiment section, authors use both a synthetic dataset and real-word datasets. However, they only compare the performance of the methods on the real-word dataset.
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} 
We report the comparison of prediction accuracy over test set on real-world datasets, which shows the practical significance of our method. Furthermore, we do not include the comparisons between InputPer and NodeDP on synthetic dataset due to the following reason. 

The experimental results on synthetic dataset has been reported in converged data pattern (Figure 7), objective convergence curves and sensitivity values (Figure 8). For InputPer, it directly adds noises on the original data and thus it is algorithmic agnostic. Therefore, it is not necessary to do comparisons over the synthetic data using the three measurements. As for NodeDP, the injected noise is highly related to the maximum degree of the node. We do not report its  result due to its high variance in a single experimental run.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $1.3$}
	The conclusion is so short that there are not any inspirations for audiences. It should present the strengths and weaknesses of the proposed method, and it is better to point out the open problems and future work.  
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} We have added the strengths and weaknesses of our method in 1st paragraph of the Conclusion section, and also discussed some open problems of designing secure metric learning models (2nd paragraph of Conclusion). For the possible future works, we refer the reviewer to Section VIII. 

The first strength lies in the novelty of the proposed problem. We study how the pairwise information could be leaked and point out the necessity of concerning the privacy for distance metric learning. The second strength is that we propose the differential pairwise privacy, a novel privacy definition for preserving pairwise data privacy via a graph perspective. The weakness of this method is that our privacy implementation is only suitable to the gradient descent based algorithms.

There are two interesting open problems that need further exploration. One is how to design a general privacy implementation method that is not limited to the exact optimization strategy. The other problem is how to use some database statistics rather than pairwise data to do distance metric learning, because it is expected to have the higher utility. 
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $1.4$}
	The references are not sufficient, some important references \cite{lee2019synthesizing, zhao2019preventing} are missing. Please cite them.  
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} These two recent papers have been properly cited in our revised version (3rd paragraph of Section II).
\hfill  $\blacksquare$

\subsection*{To Reviewer \#2}
Thank you very much for your kind comments. Below is a report for how we address your concerns. 
%% -------------------------------------------------------------------------
\begin{shaded}
	\noindent \textbf{Comment $2.1$}
	The text ``Prior knowledge" in Figure 3 is not readable well. 
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} Sorry for making this unreadable in Figure 3. ``Prior knowledge" is the knowledge about the database that the attacker has already known before attacking. It is first introduced in the 3rd paragraph of Introduction and has been used in both Figures 1 and 2. We have rewritten the caption of Figure 3 to make it clearer.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $2.2$}
	The ``green" and ``red" lines in Figure 5 can not be seen in black/white format. 
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} Thanks for pointing this out. In the revised version, an alternative way is used to mark the two disjoint paths in Figure 5. We have also carefully checked and modified other figures.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $2.3$}
	Figure 2 is not self-explanatory. Please explain it better in the caption or clarify the pictures. 
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:}  We have rewritten the caption of Figure 2 and added more explanations in the 5th paragraph of the Introduction.

In the caption, we have clarified that bottom-left prior knowledge presents one of the possible worst cases. This prior knowledge is fed into the randomized distance metric learning model and is expected to have the similar output ($M_0$) with the original dataset ($M_1$). On the one hand, $M_0$ is statistically close to $M_1$. As a convention, ``Hardly distinguishable" is used following the terminology of Dwork et al \cite{dwork2006calibrating}. On the other hand, $M_0$ is supposed to group training data in projected space as $M_1$ does. This is required by the idea of distance metric learning.

In the text, we have made clear that the pairwise data altogether can be viewed as a graph, and the differences between the original data and prior knowledge are a number of edges on the graph. This also reminds readers that some graph properties will be later leveraged in our main method.
\hfill  $\blacksquare$


\subsection*{To Reviewer \#3}
Thanks for your valuable comments. Below is a report for how we address your main concerns. For minor typos, we have corrected them one by one in the revised paper.
%% -------------------------------------------------------------------------
\begin{shaded}
	\noindent \textbf{Comment $3.1$}
	The idea of protecting the edges of a graph, instead of the nodes is not novel. There are several papers \cite{nissim2007smooth,karwa2011private,hay2009accurate,rastogi2009relationship,zhang2015private} about edge differential privacy that are not considered in the paper.
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} The novelty of this work lies in that pairwise data are modeled using graph edges so that the graph properties can be used to reveal the involved pair correlations. This is different from the conventional edge differential privacy where edge relations are not concerned.  

We notice that the mentioned works by the reviewer focuses on studying the graph statistics, such as subgraph counting \cite{karwa2011private, zhang2015private}, node degree distribution \cite{hay2009accurate}, or path length distribution \cite{rastogi2009relationship}. Paper \cite{nissim2007smooth} provides a general framework of releasing some aggregated information of database while preserving the individual privacy. However, in our work, pairwise data for the distance metric learning is formatted as graph, then the transitivity issues through edges are studied to remain the pairwise privacy during model training. We have properly cited the above works in the revised version.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $3.2$}
	The security model is not clear. If I have well understood, there is a database owner that knows which class each node belongs to and can compute the distances between nodes. The attacker knows a subset of such information. The system should prevent that the attacker infers other information. The idea is to transform the problem of node protection in the problem of distance protection. However, it is unrealistic that the attacker knows some distances without knowing the relative information of the node. Hence I observe a duality between the two problems. Authors should better clarify the security model and also compare the pairwise differential privacy problem on a secure metric with a classical node differential privacy problem.
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} Sorry for confusing the reviewer about the secure model. We have added more explanations to clarify the secure model and put more efforts to differentiate with the edge/node differential privacy.

First of all, we would clarify the specific type of the data that a database owner has. As we stated in the Notation, the database comprises $K$ pairwise data, each of which is a tuple with element being feature difference $\Delta x_{ij}$ and pairwise label $y_{ij}$. $y_{ij}$ is a binary variable which indicates if $i$ and $j$ are from same class or not. In the Introduction, we have shown such a setting is corresponding to some real-world applications. For example, in healthcare data \cite{wang2011integrating,huai2018uncorrelated}, doctors just give that two candidates the same disease probably by considering their similar symptoms and similar medical test results. Again, in our setting, only their differences and pairwise labels are recorded in database. This is reasonable because metric learning model is trained without need seeing each raw feature. This is different from classification where every sample has an exact class label. We can say that classification-like setting serves as a sufficient condition of pairwise labelled data. Please note the total class number for pairwise data could be absent. 

Second, we differentiate the proposed differential pairwise privacy with edge differential privacy and node differential privacy. 1) Edge. As shown on the right side of Figure 4, pairwise data actually corresponds to the edges of a graph while nodes only keep their identities. That means all the useful information for model training (see Eq. (7)) is on the edges of the graph. Suppose the attacker wants to know if person A and B are similar or not. Apparently, it can be answered by the edge information. However, as we analyzed in the 4th paragraph of Introduction, (edge) differential privacy is not enough to preserve the pairwise data because of the transitivity issues (see example in 4th paragraph of Introduction). Thus we need to hide more edges instead of only the one between person A and B. 2) Node. Node differential privacy tries to hide every node in the graph. This definition can be used to solve the aforementioned attack problem. However, please note when a node is added or deleted, all the edges attached to the node should also be added or deleted. For the worst case, the involved edge number should equal to the maximum node degree. Therefore, the privacy cost for node differential privacy is high. A statistic connection between node differential privacy and our privacy definition is shown in the last paragraph of Appendix A.

%As referred at the end of Section V, the proposed privacy definition is able to bear the individual participation. That means we allow the attacker to know the participation of the two persons, i.e., the existence of these two nodes. But for node differential privacy, the existence of every node is hidden. If a node is removed or added, the attached edges will be affected. Thus, in our problem, the privacy cost of node differential privacy will be high.  

The node differential privacy implementation in our experiments follows the idea of \cite{kasiviswanathan2013analyzing}. This is embedded into gradient perturbation during algorithm optimization.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $3.3$} 
	The database owner knows the class each node belongs to, hence it can compute the distance between any couple of nodes. Hence the obtained graph is fully connected. This is not considered in the paper. Does it have some impact on the proposed solution, and in the allowed attacker prior knowledge G'?
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} From our analysis in the Comment 3.2, the obtained graph is usually not fully connected. Actually, in distance metric learning, the number of pairwise data $K$ is much smaller than $\frac{n(n-1)}{2}$, where $n$ is the number of samples. For one reason, pairwise labeling is expensive in real world. For another  reason, the distance metric could be learned without too many pairs empirically. 
% For some extreme case, e.g., the obtained graph is fully connected, there will be a great number of transitivity clues for inference. Then the proposed privacy definition will be downgraded into node differential privacy, and the prior knowledge $G'$ is a subset containing $\frac{(n-1)(n-2)}{2}$ pairs. However, this will lead to a large perturbation on gradient, and the utility of output distance metric might be low.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $3.5$}
     Three minor concerns. (a) Section II.B. Methods description is too short and does not provide any useful information. (b) \cite{zhang2017efficient} is in both output perturbation and gradient perturbation, is it correct? (c) In Figure 7, why do the plots show the results applied to the original data in the database instead of the $(\Delta x, y)$ couples?
\end{shaded}
\vspace{1mm}
 \noindent \textbf{Response:} (a) We have extended methods description and introduced a privacy implementation recipe for gradient perturbation approach in Section II. B. (b) It is correct. The involved work \cite{zhang2017efficient} presents both an output perturbation and a gradient perturbation algorithm. (c) Sorry for confusing the reviewer about this. As a convention in distance metric learning, if the original data is accessible, their data pattern in the projected space can be used to verify whether the algorithms can well fit the training data. The original data is not accessible in real world, and we have added this claim in the revised version.
\hfill  $\blacksquare$

==> R1.tex <==
% !TEX root = response.tex

\newpage
\subsection*{To Reviewer \#1}
Thank you very much for such valuable comments. Below is a report for how we address your concerns. 
%% -------------------------------------------------------------------------
\begin{shaded}
	\noindent \textbf{Comment $1.1$}
	In Introduction Section, the authors did not mention graphs. However, in Section III, the Notation and the definition are based on the graph structure. Please introduce the graph structure to readers in the Introduction Section. 
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} We have introduced the graph structure in the 5th paragraph of the Introduction section as suggested by the reviewer. Given a number of pairwise data, we can describe them on a indirect graph. Then the pairwise information can be naturally encoded on edges. This is the base of our method, and we thank the reviewer for pointing this out.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $1.2$}
	In the experiment section, authors use both a synthetic dataset and real-word datasets. However, they only compare the performance of the methods on the real-word dataset.
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} 
We report the comparison of prediction accuracy over test set on real-world datasets, which shows the practical significance of our method. Furthermore, we do not include the comparisons between InputPer and NodeDP on synthetic dataset due to the following reason. 

The experimental results on synthetic dataset has been reported in converged data pattern (Figure 7), objective convergence curves and sensitivity values (Figure 8). For InputPer, it directly adds noises on the original data and thus it is algorithmic agnostic. Therefore, it is not necessary to do comparisons over the synthetic data using the three measurements. As for NodeDP, the injected noise is highly related to the maximum degree of the node. We do not report its  result due to its high variance in a single experimental run.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $1.3$}
	The conclusion is so short that there are not any inspirations for audiences. It should present the strengths and weaknesses of the proposed method, and it is better to point out the open problems and future work.  
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} We have added the strengths and weaknesses of our method in 1st paragraph of the Conclusion section, and also discussed some open problems of designing secure metric learning models (2nd paragraph of Conclusion). For the possible future works, we refer the reviewer to Section VIII. 

The first strength lies in the novelty of the proposed problem. We study how the pairwise information could be leaked and point out the necessity of concerning the privacy for distance metric learning. The second strength is that we propose the differential pairwise privacy, a novel privacy definition for preserving pairwise data privacy via a graph perspective. The weakness of this method is that our privacy implementation is only suitable to the gradient descent based algorithms.

There are two interesting open problems that need further exploration. One is how to design a general privacy implementation method that is not limited to the exact optimization strategy. The other problem is how to use some database statistics rather than pairwise data to do distance metric learning, because it is expected to have the higher utility. 
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $1.4$}
	The references are not sufficient, some important references \cite{lee2019synthesizing, zhao2019preventing} are missing. Please cite them.  
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} These two recent papers have been properly cited in our revised version (3rd paragraph of Section II).
\hfill  $\blacksquare$

\subsection*{To Reviewer \#2}
Thank you very much for your kind comments. Below is a report for how we address your concerns. 
%% -------------------------------------------------------------------------
\begin{shaded}
	\noindent \textbf{Comment $2.1$}
	The text ``Prior knowledge" in Figure 3 is not readable well. 
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} Sorry for making this unreadable in Figure 3. ``Prior knowledge" is the knowledge about the database that the attacker has already known before attacking. It is first introduced in the 3rd paragraph of Introduction and has been used in both Figures 1 and 2. We have rewritten the caption of Figure 3 to make it clearer.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $2.2$}
	The ``green" and ``red" lines in Figure 5 can not be seen in black/white format. 
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} Thanks for pointing this out. In the revised version, an alternative way is used to mark the two disjoint paths in Figure 5. We have also carefully checked and modified other figures.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $2.3$}
	Figure 2 is not self-explanatory. Please explain it better in the caption or clarify the pictures. 
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:}  We have rewritten the caption of Figure 2 and added more explanations in the 5th paragraph of the Introduction.

In the caption, we have clarified that bottom-left prior knowledge presents one of the possible worst cases. This prior knowledge is fed into the randomized distance metric learning model and is expected to have the similar output ($M_0$) with the original dataset ($M_1$). On the one hand, $M_0$ is statistically close to $M_1$. As a convention, ``Hardly distinguishable" is used following the terminology of Dwork et al \cite{dwork2006calibrating}. On the other hand, $M_0$ is supposed to group training data in projected space as $M_1$ does. This is required by the idea of distance metric learning.

In the text, we have made clear that the pairwise data altogether can be viewed as a graph, and the differences between the original data and prior knowledge are a number of edges on the graph. This also reminds readers that some graph properties will be later leveraged in our main method.
\hfill  $\blacksquare$


\subsection*{To Reviewer \#3}
Thanks for your valuable comments. Below is a report for how we address your main concerns. For minor typos, we have corrected them one by one in the revised paper.
%% -------------------------------------------------------------------------
\begin{shaded}
	\noindent \textbf{Comment $3.1$}
	The idea of protecting the edges of a graph, instead of the nodes is not novel. There are several papers \cite{nissim2007smooth,karwa2011private,hay2009accurate,rastogi2009relationship,zhang2015private} about edge differential privacy that are not considered in the paper.
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} The novelty of this work lies in that pairwise data are modeled using graph edges so that the graph properties can be used to reveal the involved pair correlations. This is different from the conventional edge differential privacy where edge relations are not concerned.  

We notice that the mentioned works by the reviewer focuses on studying the graph statistics, such as subgraph counting \cite{karwa2011private, zhang2015private}, node degree distribution \cite{hay2009accurate}, or path length distribution \cite{rastogi2009relationship}. Paper \cite{nissim2007smooth} provides a general framework of releasing some aggregated information of database while preserving the individual privacy. However, in our work, pairwise data for the distance metric learning is formatted as graph, then the transitivity issues through edges are studied to remain the pairwise privacy during model training. We have properly cited the above works in the revised version.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $3.2$}
	The security model is not clear. If I have well understood, there is a database owner that knows which class each node belongs to and can compute the distances between nodes. The attacker knows a subset of such information. The system should prevent that the attacker infers other information. The idea is to transform the problem of node protection in the problem of distance protection. However, it is unrealistic that the attacker knows some distances without knowing the relative information of the node. Hence I observe a duality between the two problems. Authors should better clarify the security model and also compare the pairwise differential privacy problem on a secure metric with a classical node differential privacy problem.
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} Sorry for confusing the reviewer about the secure model. We have added more explanations to clarify the secure model and put more efforts to differentiate with the edge/node differential privacy.

First of all, we would clarify the specific type of the data that a database owner has. As we stated in the Notation, the database comprises $K$ pairwise data, each of which is a tuple with element being feature difference $\Delta x_{ij}$ and pairwise label $y_{ij}$. $y_{ij}$ is a binary variable which indicates if $i$ and $j$ are from same class or not. In the Introduction, we have shown such a setting is corresponding to some real-world applications. For example, in healthcare data \cite{wang2011integrating,huai2018uncorrelated}, doctors just give that two candidates the same disease probably by considering their similar symptoms and similar medical test results. Again, in our setting, only their differences and pairwise labels are recorded in database. This is reasonable because metric learning model is trained without need seeing each raw feature. This is different from classification where every sample has an exact class label. We can say that classification-like setting serves as a sufficient condition of pairwise labelled data. Please note the total class number for pairwise data could be absent. 

Second, we differentiate the proposed differential pairwise privacy with edge differential privacy and node differential privacy. 1) Edge. As shown on the right side of Figure 4, pairwise data actually corresponds to the edges of a graph while nodes only keep their identities. That means all the useful information for model training (see Eq. (7)) is on the edges of the graph. Suppose the attacker wants to know if person A and B are similar or not. Apparently, it can be answered by the edge information. However, as we analyzed in the 4th paragraph of Introduction, (edge) differential privacy is not enough to preserve the pairwise data because of the transitivity issues (see example in 4th paragraph of Introduction). Thus we need to hide more edges instead of only the one between person A and B. 2) Node. Node differential privacy tries to hide every node in the graph. This definition can be used to solve the aforementioned attack problem. However, please note when a node is added or deleted, all the edges attached to the node should also be added or deleted. For the worst case, the involved edge number should equal to the maximum node degree. Therefore, the privacy cost for node differential privacy is high. A statistic connection between node differential privacy and our privacy definition is shown in the last paragraph of Appendix A.

%As referred at the end of Section V, the proposed privacy definition is able to bear the individual participation. That means we allow the attacker to know the participation of the two persons, i.e., the existence of these two nodes. But for node differential privacy, the existence of every node is hidden. If a node is removed or added, the attached edges will be affected. Thus, in our problem, the privacy cost of node differential privacy will be high.  

The node differential privacy implementation in our experiments follows the idea of \cite{kasiviswanathan2013analyzing}. This is embedded into gradient perturbation during algorithm optimization.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $3.3$} 
	The database owner knows the class each node belongs to, hence it can compute the distance between any couple of nodes. Hence the obtained graph is fully connected. This is not considered in the paper. Does it have some impact on the proposed solution, and in the allowed attacker prior knowledge G'?
\end{shaded}
\vspace{1mm}
\noindent \textbf{Response:} From our analysis in the Comment 3.2, the obtained graph is usually not fully connected. Actually, in distance metric learning, the number of pairwise data $K$ is much smaller than $\frac{n(n-1)}{2}$, where $n$ is the number of samples. For one reason, pairwise labeling is expensive in real world. For another  reason, the distance metric could be learned without too many pairs empirically. 
% For some extreme case, e.g., the obtained graph is fully connected, there will be a great number of transitivity clues for inference. Then the proposed privacy definition will be downgraded into node differential privacy, and the prior knowledge $G'$ is a subset containing $\frac{(n-1)(n-2)}{2}$ pairs. However, this will lead to a large perturbation on gradient, and the utility of output distance metric might be low.
\hfill  $\blacksquare$

\begin{shaded}
	\noindent \textbf{Comment $3.5$}
     Three minor concerns. (a) Section II.B. Methods description is too short and does not provide any useful information. (b) \cite{zhang2017efficient} is in both output perturbation and gradient perturbation, is it correct? (c) In Figure 7, why do the plots show the results applied to the original data in the database instead of the $(\Delta x, y)$ couples?
\end{shaded}
\vspace{1mm}
 \noindent \textbf{Response:} (a) We have extended methods description and introduced a privacy implementation recipe for gradient perturbation approach in Section II. B. (b) It is correct. The involved work \cite{zhang2017efficient} presents both an output perturbation and a gradient perturbation algorithm. (c) Sorry for confusing the reviewer about this. As a convention in distance metric learning, if the original data is accessible, their data pattern in the projected space can be used to verify whether the algorithms can well fit the training data. The original data is not accessible in real world, and we have added this claim in the revised version.
\hfill  $\blacksquare$
